Backdoor Scanning for Deep Neural Networks through K-Arm Optimization

Back-door attack poses a severe threat to deep learning systems. It injects hidden malicious behaviors to a model such that any input stamped with a special pattern can trigger such behaviors. Detecting back-door is hence of pressing need. Many existing defense techniques use optimization to generate the smallest input pattern that forces the model to misclassify a set of benign inputs injected with the pattern to a target label. However, the complexity is quadratic to the number of class labels such that they can hardly handle models with many classes. Inspired by Multi-Arm Bandit in Reinforcement Learning, we propose a K-Arm optimization method for backdoor detection. By iteratively and stochastically selecting the most promising labels for optimization with the guidance of an objective function, we substantially reduce the complexity, allowing to handle models with many classes. Moreover, by iteratively refining the selection of labels to optimize, it substantially mitigates the uncertainty in choosing the right labels, improving detection accuracy. At the time of submission, the evaluation of our method on over 4000 models in the IARPA TrojAI competition from round 1 to the latest round 4 achieves top performance on the leaderboard. Our technique also supersedes three state-of-the-art techniques in terms of accuracy and the scanning time needed.

==> Table&Algorithm/Imagenet.tex <==
\begin{table}[t]
\caption{Imagenet}
%Attack success rate remain 0\% even when we set bound size to 32. We adjust the hyper-parameter of adversarial loss item in AdvGAN's objective function to -100 for the untarget attack and AdvGAN still shows lower attack success rate and less mIoU drop than our AdvSAPDE( 7.8\% attack success rate when bound size is 8). The result proves that AdvGAN is designed for classification task and not effective for segmentation task.

\label{Imagenet}
\centering
\scalebox{0.95}{
\scriptsize
\begin{tabular}{lrr}
\toprule
%\multicolumn{4}{c}{DRN-105} \\
%\midrule
Methods        &Detection Acc     &Avg Time\\
\midrule
ABS &100\%     &4920s     \\
NC   &75\% &221341s  \\
Low-cost NC &62.5\%     &42020s     \\
\textbf{K-Arm Opt}  &\textbf{87.5\%}         &\textbf{19800s}       \\
\textbf{K-Arm+Arm Reduction}  &\textbf{100\%}    &\textbf{224s}     \\

\bottomrule
\end{tabular}
}
\end{table}

==> Table&Algorithm/algorithm.tex <==
\begin{algorithm}[H]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\Input{Model $\mathcal F$, Sample inputs $X_i$ for each class $i$.}
\KwResult{Trigger Size $s$, Victim label $v$,  Target label $t$ }
%\KwResult{Prediction $p$}

 victims $V$, targets $T$ = Pre-Screening($\mathcal F$, $X$)
 
  \uIf{$V$ != None}{
    initialization: Masks $M_i$, Patterns $P_i$ for each $i$ in $V$
    
    %$M^\prime$, $P^\prime$ = 
    Warm-Up($\mathcal F$, $X$,$M$,$P$)
    
    Update(M,P)
    
    \While{i \le Rounds}{
    $v$,$t$ = K\_Arm\_scheduler($M$, $P$)
    
    %$m^\prime$,$p^\prime$ = 
    Trigger\_Optimization($\mathcal F$,$X_v$,$t$,$M_v$,$P_v$)

    Symmetric\_Trigger\_Optimization($\mathcal F$,$X_t$,$v$,$M_t$,$P_t$)
    
    Update(M,P)
    
    }
    
    idx = argmin(M)
    
    trigger\_size s = \min(|$M$|_1)
    
    victim\_label $v$ = $V_{idx}$
    
    target\_label $t$ = $T_{idx}$
    
    return $s, v, t$
    
}
 %initialization\: 

 \caption{Symmetric K-Arm Optimization}
\end{algorithm}

==> Table&Algorithm/dataset.tex <==



\begin{table*}[t]
\caption{TrojAI Dataset} 
%\vspace{-10pt}
% ($84.4\%$ on Cityscapes, $57.7\%$ on ADE20K) than traditional norm-bounded attack approaches, as shown in Table~\ref{Success Rate}. 
% The results show that PGD and FGSM attacks can barely attack target networks with small bound size ($\epsilon = 0.25,1,8$). 
% For instance, FGSM attack with bound size $\epsilon = 1$ on real and vanilla SPADE generated images achieve $0\%$ attack success rate on DRN-105 network on Cityscapes. In contrast, AdvSPADE achieves high attack success rate ($84.4\%$ and $57.7\%$ on DRN-105 and Upernet-101, respectively).
\label{dataset}
\centering
\scalebox{0.65}{
\footnotesize
%\small
\tabcolsep=4pt
%\begin{tabular}{lcccc}
\begin{tabular}{l|rrrrrrrrrr}
\toprule
Rounds      &\# of Models    &\# of Classes     &\# of Samples per Class    &\# of Model Architectures   &\# of Triggers  &Global Trigger   &Label-specific Trigger     &Polygon Trigger  &Instagram Filter Trigger     &Adv.Training   \\
\midrule

Round1  &1000   &5      &100    &3  &1  &\ding{51}     &\ding{55}   &\ding{51}  &\ding{55} &\ding{55}  \\

Round2  &1104   &5$\sim$25      &10$\sim$20    &23  &1   &\ding{51}     &\ding{51}   &\ding{51}  &\ding{51} &\ding{55}  \\

Round3  &1008   &5$\sim$25       &10$\sim$20    &23  &1     &\ding{51}     &\ding{51}   &\ding{51}  &\ding{51} &\ding{51}  \\

Round4  &1008   &15$\sim$44       &2$\sim$5    &16  &1$\sim$2   &\ding{55}     &\ding{51}   &\ding{51}  &\ding{51} &\ding{51}  \\


%\midrule
%Clean Image &0\%    &0.756    &-
%&Clean Image &0\%   &0.420    &- \\

%Vanilla SPADE   &0\%    &0.620  &62.939
%&Vanilla SPADE  &0\%    &0.403  &33.9 \\


%          &22.2\%   &0.036   &-    &~30s/Image  
%&          &11.5\%   &0.070  &-    &~34s/Image \\

                        



%\bf{Ours}         &\bf{84.4\%  }  &\bf{0.01  }    &\bf{67.302}  &\bf{0.25s/Image} &\bf{Ours}     &\bf{57.7\%}   &\bf{0.011 }   &\bf{53.49}  &\bf{0.32s/Image}\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table*}


==> Table&Algorithm/karm_roun1_1000.tex <==
\begin{table}[h]
\caption{Results on round1 1000 models} 
% ($84.4\%$ on Cityscapes, $57.7\%$ on ADE20K) than traditional norm-bounded attack approaches, as shown in Table~\ref{Success Rate}. 
% The results show that PGD and FGSM attacks can barely attack target networks with small bound size ($\epsilon = 0.25,1,8$). 
% For instance, FGSM attack with bound size $\epsilon = 1$ on real and vanilla SPADE generated images achieve $0\%$ attack success rate on DRN-105 network on Cityscapes. In contrast, AdvSPADE achieves high attack success rate ($84.4\%$ and $57.7\%$ on DRN-105 and Upernet-101, respectively).
\label{karm_1000}
\centering

\scalebox{0.7}{
\footnotesize
%\begin{tabular}{lcccc}
\begin{tabular}{l|rrrr}
\toprule
 &\multicolumn{4}{c}{Round1 Trainset (1000)} \\
\midrule
Method      &Acc &Loss   &ROC   &Time   \\

%\midrule
%Clean Image &0\%    &0.756    &-
%&Clean Image &0\%   &0.420    &- \\

%Vanilla SPADE   &0\%    &0.620  &62.939
%&Vanilla SPADE  &0\%    &0.403  &33.9 \\

\midrule
\textbf{K-Arm Opt}  &\textbf{91}\%   &\textbf{0.31}   &\textbf{0.90}    &\textbf{265.5s}    \\ 
%          &22.2\%   &0.036   &-    &~30s/Image  
%&          &11.5\%   &0.070  &-    &~34s/Image \\

                        



%\bf{Ours}         &\bf{84.4\%  }  &\bf{0.01  }    &\bf{67.302}  &\bf{0.25s/Image} &\bf{Ours}     &\bf{57.7\%}   &\bf{0.011 }   &\bf{53.49}  &\bf{0.32s/Image}\\
\bottomrule
\end{tabular}
\vspace{-10mm}
}
\end{table}

